All CAT(0) Boundaries of a Group of the Form HxK are CE Equivalent

M. Bestvina has shown that for any given torsion-free CAT(0) group G, all of its boundaries are shape equivalent. He then posed the question of whether they satisfy the stronger condition of being cell-like equivalent. In this article we prove that the answer is "Yes" in the situation where the group in question splits as a direct product with infinite factors. We accomplish this by proving an interesting theorem in shape theory.

==> biblio.tex <==
\begin{thebibliography}{999}

\bibitem[AGW]{AGW} F.D. Ancel, C. Guilbault, and J. Wilson,
	\emph{The Croke-Kleiner boundaries are cell-like equivalent,}
	Preprint.

\bibitem[Be]{Be} M. Bestvina,
	\emph{Local homology properties of boundaries of groups,}
	Michigan Math. J. 43 (1996), no. 1, 123-139.

\bibitem[BH]{BH} M.R. Bridson and A. Haefliger,
	\emph{Metric Spaces of Nonpositive Curvature,}
	Springer-Verlag, Berlin, 1999.

\bibitem[Bo]{Bo} K. Borsuk,
	\emph{Theory of Shape,}
	Mathematical Monographs, Vol. 59, Polish Scientific Publishing House, Warsaw. (1975).

\bibitem[BR]{BR} P.L. Bowers and K. Ruane,
	\emph{Boundaries of nonpositively curved groups of the form \(G\times\mathbb{Z}\),}
	Glasgow Math. J. 38 (1996), 177-189.

\bibitem[Ch]{Ch} T.A. Chapman,
	\emph{Lectures on Hilbert cube manifolds,}
	C.B.M.S. Regional Conf. Series in Math. 28, 1976.

\bibitem[Ch2]{Ch2} T.A. Chapman,
	\emph{Shapes of finite-dimensional compacta,}
	Fund. Math. 76 (1972), 329-353.

\bibitem[CK]{CK} C. Croke and B. Kleiner,
	\emph{Spaces with nonpositive curvature and their ideal boundaries,}
	Topology 39 (2000), no. 3, 549-556.

\bibitem[CK2]{CK2} C. Croke and B. Kleiner,
	\emph{The geodesic flow of a nonpositively curved graph manifold,}
	Geom. Funct. Anal. 12 (2002), no. 3, 479--545.

\bibitem[Da]{Da} R. J. Daverman,
	\emph{Decompositions of manifolds,}
	Pure and Applied Mathematics, 124. Academic Press, Inc., Orlando, FL, 1986. xii+317 pp.

\bibitem[Fe]{Fe} S. Ferry,
	\emph{Homotopy, simple homotopy, and compacta,}
	Topology 19 (1980), no. 2, 101--110.

\bibitem[Fe2]{Fe2} S. Ferry,
	\emph{Shape Equivalence does not Imply CE Equivalence,}
	Proc. Amer. Math. Soc. 80 (1980), no. 1, 1980 154--156.

\bibitem[Has]{Has}
	\emph{Suspensions of strong shape equivalences are CE equivalences,}
	Proc. Amer. Math. Soc. 87 (1983), no. 4, 743--745.

\bibitem[Ho]{Ho} T. Hosaka,
	\emph{On splitting theorems for CAT(0) spaces and compact geodesic spaces of non-positive curvature,}
	Preprint, arXiv:math/0405551.

\bibitem[Hr]{Hr} C. Hruska,
	\emph{Geometric invariants of spaces with isolated flats,}
	Topology 44 (2005), no. 2, 441--458. 

\bibitem[HW]{HW} W. Hurewicz and H. Wallman,
	\emph{Dimension Theory,}
	Princeton University Press, Princeton, 1969.

\bibitem[Mo]{Mo} C. Mooney,
	\emph{Examples of Non-Rigid CAT(0) Groups from the Category of Knot Groups,}
	Preprint, arXiv:math/0706.1581.

\bibitem[Mo2]{MoCK} C. Mooney,
	\emph{Generalizing the Croke-Kleiner Construction,}
	Preprint.

\bibitem[Mu]{Mu} J. R. Munkres,
	\emph{Topology, 2nd Ed,}
	Prentice-Hall, Inc., Upper Saddle River, N.J., 2000.

\bibitem[MS]{MS} S. Marde\v{s}i\'{c} and J. Segal,
	\emph{Shape Theory,}
	North-Holland, Amsterdam (1982).

\bibitem[On]{On} P. Ontaneda,
	\emph{Cocompact CAT(0) Spaces are Almost Geodesically Complete,}
	Topology 44 (2005), no. 1, 47--62.

\bibitem[Ru]{Ru} K. Ruane,
	\emph{Boundaries of CAT(0) groups of the form \(\Gamma=G\times H\),}
	Topology Appl. 92 (1999), 131-152.

\bibitem[Sh]{Sh} R. B. Sher,
	\emph{Realizing cell-like maps in Euclidean space,}
	General Topology and Appl. 2 (1972), 75--89.

\bibitem[Sw]{Sw} E. L. Swenson,
	\emph{A cut point theorem for CAT(0) groups,}
	Jour. Diff. Geom. 53 (1999) 327-358.

\bibitem[Ta]{Ta} J. Taylor,
	\emph{A counterexample in shape theory,}
	Bull. Amer. Math. Soc. 81 (1975), 629--632.

\bibitem[Ve]{Ve} G. Venema,
	\emph{Embeddings of compacta with shape dimension in the trivial range,}
	Proc. A.M.S. (1976).

\bibitem[Wi]{Wi} J.M. Wilson,
	\emph{A CAT(0) group with uncountably many distinct boundaries,}
	J. Group Theory 8 (2005), no. 2, 229--238.

\end{thebibliography}


==> rightarrow.tex <==
\beginpicture
\setcoordinatesystem units <0.28146cm,0.28146cm>
\put {\phantom{.}} at -2.09358 -1.11646
\put {\phantom{.}} at -2.09358 1.11646
\put {\phantom{.}} at 1.45928 -1.11646
\put {\phantom{.}} at 1.45928 1.11646
\setlinear
\setshadesymbol <z,z,z,z> ({\fiverm .})
\plot 1.00000 0.00000 0.00000 1.00000 /
\putrule from 1.00000 0.00000 to -2.00000 0.00000
\plot 1.00000 0.00000 0.00000 -1.00000 /
\endpicture

